ALIP: Adaptive Language-Image Pre-training with Synthetic Caption

Contrastive Language-Image Pre-training (CLIP) has significantly boosted the performance of various vision-language tasks by scaling up the dataset with image-text pairs collected from the web. However, the presence of intrinsic noise and unmatched image-text pairs in web data can potentially affect the performance of representation learning. To address this issue, we first utilize the OFA model to generate synthetic captions that focus on the image content. The generated captions contain complementary information that is beneficial for pre-training. Then, we propose an Adaptive Language-Image Pre-training (ALIP), a bi-path model that integrates supervision from both raw text and synthetic caption. As the core components of ALIP, the Language Consistency Gate (LCG) and Description Consistency Gate (DCG) dynamically adjust the weights of samples and image-text/caption pairs during the training process. Meanwhile, the adaptive contrastive loss can effectively reduce the impact of noise data and enhances the efficiency of pre-training data. We validate ALIP with experiments on different scales of models and pre-training datasets. Experiments results show that ALIP achieves state-of-the-art performance on multiple downstream tasks including zero-shot image-text retrieval and linear probe. To facilitate future research, the code and pre-trained models are released at https://github.com/deepglint/ALIP.

==> table/imagenet_classification.tex <==

\begin{table}[h]
\caption{Full ImageNet results.
SLIP significantly improves performance on ImageNet in the zero-shot transfer, linear classification, and end-to-end finetuning settings.}
\label{tab:table1}
\begin{tabular}{l l l l l}
    \toprule
    Model & Method & 0-shot & Linear & Finetuned \\
    \midrule
    RN50 & CLIP & \underline{32.7} & \underline{59.3} & 78.2 \\
     & Our & \textbf{38.3} (+5.6) & \textbf{66.4} (+7.1) & \textbf{80.3} (+0.4) \\
    \midrule
    RN101 & CLIP & \underline{37.6} & \underline{66.5} & 80.5 \\
     & Our & \textbf{42.8} (+5.2) & \textbf{72.1} (+5.6) & \textbf{82.6} (+0.1) \\
    \midrule
    ViT B/32 & CLIP & \underline{37.6} & \underline{66.5} & 80.5 \\
     & Our & \textbf{42.8} (+5.2) & \textbf{72.1} (+5.6) & \textbf{82.6}  \\
    \midrule
    ViT B/16 & CLIP & \underline{40.4} & \underline{70.5} & 81.0 \\
     & Our & \textbf{46.2} (+4.8) & \textbf{76.0} (+5.5) & \textbf{84.2} \\
     \bottomrule
\end{tabular}

\end{table}


==> table/linear_prob.tex <==
\begin{table*}
	\caption{Top-1 accuracy(\%) of linear probe on 26 image classification datasets. }
	\label{tab:linear-probe-big-table}
	\centering
	\resizebox{1.0\linewidth}{!}{
		\begin{tabular}{cl|ccccccccccccccccccccccccccc|c}
			\toprule
			 &              &  & \rotatebox[origin=lb]{90}{\smash{Food101}} & \rotatebox[origin=lb]{90}{\smash{CIFAR10}} & \rotatebox[origin=lb]{90}{\smash{CIFAR100}} & \rotatebox[origin=lb]{90}{\smash{Birdsnap}} & \rotatebox[origin=lb]{90}{\smash{SUN397}} & \rotatebox[origin=lb]{90}{\smash{Cars}} & \rotatebox[origin=lb]{90}{\smash{Aircraft}} & \rotatebox[origin=lb]{90}{\smash{voc2007}} & \rotatebox[origin=lb]{90}{\smash{DTD}} & \rotatebox[origin=lb]{90}{\smash{Pets}} & \rotatebox[origin=lb]{90}{\smash{Caltech101}} & \rotatebox[origin=lb]{90}{\smash{Flowers}} & \rotatebox[origin=lb]{90}{\smash{MNIST}} & \rotatebox[origin=lb]{90}{\smash{FER2013}} & \rotatebox[origin=lb]{90}{\smash{STL10}} & \rotatebox[origin=lb]{90}{\smash{EuroSAT}} & \rotatebox[origin=lb]{90}{\smash{RESISC45}} & \rotatebox[origin=lb]{90}{\smash{GTSRB}} & \rotatebox[origin=lb]{90}{\smash{KITTI}} & \rotatebox[origin=lb]{90}{\smash{Country211}} & \rotatebox[origin=lb]{90}{\smash{PCAM}} & \rotatebox[origin=lb]{90}{\smash{UCF101}} & \rotatebox[origin=lb]{90}{\smash{Kinetics700}} & \rotatebox[origin=lb]{90}{\smash{CLEVR}} & \rotatebox[origin=lb]{90}{\smash{HatefulMemes}} & \rotatebox[origin=lb]{90}{\smash{SST}} & \rotatebox[origin=lb]{90}{\smash{Average}} \\
			
			\midrule \multirow{8}{3em}{\rotatebox[origin=c]{90}{Laion 10M}}
   
			 & CLIP RN50     &  & 95.1   & 80.5  & 93.0  & 81.8  & 96.9  & 88.8  & 58.5  & 76.6  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8 & 81.8   \\    

              & Our RN50     &  & 95.1   & 80.5  & 93.0  & 81.8  & 96.9  & 88.8  & 58.5  & 76.6  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8 & 81.8   \\   

               & CLIP RN101     &  & 95.1   & 80.5  & 93.0  & 81.8  & 96.9  & 88.8  & 58.5  & 76.6  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8 & 81.8   \\    

              & Our RN101     &  & 95.1   & 80.5  & 93.0  & 81.8  & 96.9  & 88.8  & 58.5  & 76.6  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8 & 81.8   \\  

              & CLIP ViT B/32     &  & 95.1   & 80.5  & 93.0  & 81.8  & 96.9  & 88.8  & 58.5  & 76.6  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8 & 81.8   \\    

              & Our ViT B/32     &  & 95.1   & 80.5  & 93.0  & 81.8  & 96.9  & 88.8  & 58.5  & 76.6  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8 & 81.8   \\   

               & CLIP ViT B/16     &  & 95.1   & 80.5  & 93.0  & 81.8  & 96.9  & 88.8  & 58.5  & 76.6  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8 & 81.8   \\    

              & Our ViT B/16     &  & 95.1   & 80.5  & 93.0  & 81.8  & 96.9  & 88.8  & 58.5  & 76.6  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8 & 81.8   \\ 
			                                
  
             \midrule \multirow{8}{3em}{\rotatebox[origin=c]{90}{Laion 30M}}
			 & Our-RN50     &  & 95.1   & 80.5  & 93.0  & 81.8  & 96.9  & 88.8  & 58.5  & 76.6  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8 & 81.8   \\  

              & Our RN50     &  & 95.1   & 80.5  & 93.0  & 81.8  & 96.9  & 88.8  & 58.5  & 76.6  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8 & 81.8   \\  

               & CLIP RN50     &  & 95.1   & 80.5  & 93.0  & 81.8  & 96.9  & 88.8  & 58.5  & 76.6  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8 & 81.8   \\    

              & Our RN101     &  & 95.1   & 80.5  & 93.0  & 81.8  & 96.9  & 88.8  & 58.5  & 76.6  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8 & 81.8   \\  

              & CLIP ViT B/32     &  & 95.1   & 80.5  & 93.0  & 81.8  & 96.9  & 88.8  & 58.5  & 76.6  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8 & 81.8   \\    

              & Our ViT B/32     &  & 95.1   & 80.5  & 93.0  & 81.8  & 96.9  & 88.8  & 58.5  & 76.6  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8 & 81.8   \\   

               & CLIP ViT B/16     &  & 95.1   & 80.5  & 93.0  & 81.8  & 96.9  & 88.8  & 58.5  & 76.6  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8 & 81.8   \\    

              & Our ViT B/16     &  & 95.1   & 80.5  & 93.0  & 81.8  & 96.9  & 88.8  & 58.5  & 76.6  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8  & 76.5  & 52.0  & 90.0  & 97.0  & 76.1  & 81.8 & 81.8   \\ 
			 
			\bottomrule
		\end{tabular}
  }
\end{table*}

==> table/text_image_retrieval.tex <==
\begin{table*}[t]
\caption{\textbf{CLIP improves zero-shot retrieval and is competitive with the best fine-tuned result on Flickr30k text retrieval.} Bold indicates best overall performance while an underline indicates best in category performance (zero-shot or fine-tuned). For all other models, best results from the paper are reported regardless of model size / variant. MSCOCO performance is reported on the 5k test set.}

\begin{tabular}{llcccccccccccc}
\toprule
& & \multicolumn{6}{c}{Text Retrieval} & \multicolumn{6}{c}{Image Retrieval} \\
& & \multicolumn{3}{c}{Flickr30k} & \multicolumn{3}{c}{MSCOCO} & \multicolumn{3}{c}{Flickr30k} & \multicolumn{3}{c}{MSCOCO} \\
& & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 \\
\midrule
\multirow{4}{3em}{\rotatebox[origin=c]{90}{Laion 10M}} 
    & CLIP RN50\ & 86.2 & 96.3 & 99.0 &  62.3 & 87.1 & 92.8 & 71.5 & 90.9 & 94.9 & 46.7 & 76.0 & 85.3 \\
    & Our RN50 & 87.3 & 98.0 & 99.2 & 65.7 & 88.6 & 93.8 & 75.6 & 94.1 & \underline{\textbf{96.8}} & 52.9 & 79.9 & 88.0 \\
    
    & CLIP RN101\ & 86.2 & 96.3 & 99.0 &  62.3 & 87.1 & 92.8 & 71.5 & 90.9 & 94.9 & 46.7 & 76.0 & 85.3 \\
    & Our RN101 & 87.3 & 98.0 & 99.2 & 65.7 & 88.6 & 93.8 & 75.6 & 94.1 & \underline{\textbf{96.8}} & 52.9 & 79.9 & 88.0 \\

\midrule
\multirow{4}{3em}{\rotatebox[origin=c]{90}{Laion 30M}} 
    & CLIP RN50\ & 86.2 & 96.3 & 99.0 &  62.3 & 87.1 & 92.8 & 71.5 & 90.9 & 94.9 & 46.7 & 76.0 & 85.3 \\
    & Our RN50 & 87.3 & 98.0 & 99.2 & 65.7 & 88.6 & 93.8 & 75.6 & 94.1 & \underline{\textbf{96.8}} & 52.9 & 79.9 & 88.0 \\
    
    & CLIP RN101\ & 86.2 & 96.3 & 99.0 &  62.3 & 87.1 & 92.8 & 71.5 & 90.9 & 94.9 & 46.7 & 76.0 & 85.3 \\
    & Our RN101 & 87.3 & 98.0 & 99.2 & 65.7 & 88.6 & 93.8 & 75.6 & 94.1 & \underline{\textbf{96.8}} & 52.9 & 79.9 & 88.0 \\
\bottomrule
\end{tabular}
\end{table*}
